Privacy in Deep Learning: A Survey

The ever-growing advances of deep learning in many areas including vision, recommendation systems, natural language processing, etc., have led to the adoption of Deep Neural Networks (DNNs) in production systems. The availability of large datasets and high computational power are the main contributors to these advances. The datasets are usually crowdsourced and may contain sensitive information. This poses serious privacy concerns as this data can be misused or leaked through various vulnerabilities. Even if the cloud provider and the communication link is trusted, there are still threats of inference attacks where an attacker could speculate properties of the data used for training, or find the underlying model architecture and parameters. In this survey, we review the privacy concerns brought by deep learning, and the mitigating techniques introduced to tackle these issues. We also show that there is a gap in the literature regarding test-time inference privacy, and propose possible future research directions.

==> body/acknowl.tex <==
\section*{Acknowledgements}
We thank Gary Marcus, Kamalika Chaudhuri, Lawrence Saul, Alex Snoeren and Dean Tullsen for insightful discussions and comments.This work was in part supported by National Science Foundation (NSF) awards CN\#1703812, ECCS\#1609823, CCF\#1553192, Air Force Office of Scientific Research (AFOSR) Young Investigator Program(YIP) award \#FA9550-17-1-0274, National Institute of Health (NIH) award \#R01EB028350, and Air Force Research Laboratory (AFRL) and Defense Advanced Research Project Agency (DARPA) under agreement number \#FA8650-20-2-7009 and \#HR0011-18-C-0020. The U.S. Government is authorized to reproduce and distribute reprints for Governmental purposes notwithstanding any copyright notation thereon. The views and conclusions contained herein are those of the authors and should not be interpreted as necessarily representing the official policies or endorsements, either expressed or implied, of NSF, AFSOR, NIH, AFRL, DARPA or the U.S. Government.
